When is Tree Search Useful for LLM Planning? It Depends on the Discriminator

In this paper, we examine how large language models (LLMs) solve multi-step problems under a language agent framework with three components: a generator, a discriminator, and a planning method. We investigate the practical utility of two advanced planning methods, iterative correction and tree search. We present a comprehensive analysis of how discrimination accuracy affects the overall performance of agents when using these two methods or a simpler method, re-ranking. Experiments on two tasks, text-to-SQL parsing and mathematical reasoning, show that: (1) advanced planning methods demand discriminators with at least 90% accuracy to achieve significant improvements over re-ranking; (2) current LLMs' discrimination abilities have not met the needs of advanced planning methods to achieve such improvements; (3) with LLM-based discriminators, advanced planning methods may not adequately balance accuracy and efficiency. For example, compared to the other two methods, tree search is at least 10--20 times slower but leads to negligible performance gains, which hinders its real-world applications. Code and data are available at https://github.com/OSU-NLP-Group/llm-planning-eval.

==> tables/gsm8k_enhanced_llm.tex <==
\begin{table}[t]
\small
\centering
\begin{tabular}{
lcccc
}
\toprule
 & \multicolumn{2}{c}{\textbf{CodeLlama-13B}} & \multicolumn{2}{c}{\textbf{GPT-3.5-Turbo}} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
 & Acc & H@1 & Acc & H@1 \\
\midrule
Naive & 62.2 & 41.8 & 72.1 & 46.6 \\
\midrule
+ Exec. Check & 64.5 & 42.6 & 73.2 & 47.6 \\
+ Exec. Result & 70.5 & \textbf{42.8} & \textbf{78.3} & \textbf{50.6} \\
+ Both & \textbf{70.6} & \textbf{42.8} & 76.5 & 48.6 \\
\midrule
Improvement & 8.4 & 1.0 & 6.3 & 4.0 \\
\bottomrule
\end{tabular}
\vspace{-6pt}
\caption{\label{tab:gsm8k_enhanced_llm}
gsm8k enhanced discriminator.
}
\vspace{-11pt}
\end{table}

==> tables/related_work.tex <==
\begin{table}[t]
%\small
\scriptsize
\centering
\begin{tabular}{
@{\hspace{0pt}}l@{\hspace{2pt}}
@{\hspace{1pt}}c@{\hspace{1pt}}
@{\hspace{1pt}}c@{\hspace{1pt}}
@{\hspace{1pt}}c@{\hspace{0pt}}
}
%{lccc}
\toprule
\multirow{2}{*}{\textbf{Comparison}} & \textbf{GenAI Paradox} & \textbf{Self-Correction} & \multirow{2}{*}{\textbf{Our Work}}\\
 & \citep{west2024paradox} & \citep{huang2024llm_selfcorrect} & \\
\midrule
% I'm trying to type as lo- & \multirow{2}{*}{\xmark} & \multirow{2}{*}{\xmark} & \multirow{2}{*}{\cmark} \\
% ng as I can &  &  &  \\
Number of Planning Me- & \multirow{2}{*}{0} & \multirow{2}{*}{1} & \multirow{2}{*}{3} \\
thods Studied & & & \\
\midrule
Open-Source LLMs & \xmark$^\dagger$ & \xmark & \cmark \\
Closed-Source LLMs & \cmark$^\dagger$ & \cmark & \cmark \\
Fine-Tuned LLMs & \xmark & \xmark & \cmark \\
\midrule
Text-to-SQL Parsing & \xmark & \xmark & \cmark \\
Mathematical Reasoning & \xmark & \cmark & \cmark \\
\bottomrule
\end{tabular}
\vspace{-6pt}
\caption{Comparison of our work to representative papers. $^\dagger$While some open-source models are evaluated for vision tasks, for language tasks, only closed-source LLMs are evaluated.}
\vspace{-11pt}
\label{tab:related_work}
\end{table}

==> tables/text2sql_bird.tex <==
\begin{table}[t]
\small
\centering
\begin{tabular}{lccc}
\toprule
\textbf{Discriminators} & \textbf{RR} & \textbf{IC} & \textbf{TS} \\
\midrule
\multicolumn{4}{c}{\textit{Naive Discriminators}} \\
\midrule
CodeLlama-13B-Instruct & 13.3 & 13.3 & 13.3 \\
GPT-3.5-Turbo &\textbf{18.0} & \textbf{17.3} & TBD \\
CodeLlama-13B-Instruct-FT & 14.3 & 13.0 & 13.0\\
\midrule
\multicolumn{4}{c}{\textit{Observation-Enhanced Discriminators}} \\
\midrule
CodeLlama-13B-Instruct & 21.0 & 24.3 & 22.7 \\
GPT-3.5-Turbo & 22.3 & 25.0 & TBD \\
CodeLlama-13B-Instruct-FT & \textbf{23.7} & \underline{\textbf{26.3}} & 21.7 \\
\midrule
\multicolumn{4}{c}{\textit{Oracle-Simulated Discriminator}} \\
\midrule
Oracle Simulation ($\tau = 1.0$) & 27.0 & 32.7 & 29.3 \\
\bottomrule
\end{tabular}
\vspace{-6pt}
\caption{\label{tab:text2sql_bird}
Text2sql Bird.
}
\vspace{-11pt}
\end{table}

==> tables/text2sql_enhanced_llm.tex <==
\begin{table*}[t]
\small
\centering
\begin{tabular}{lcccccccccccc}
\toprule

 & \multicolumn{4}{c}{\textbf{CodeLlama-13B}} & \multicolumn{4}{c}{\textbf{GPT-3.5-Turbo}} & \multicolumn{4}{c}{\textbf{CodeLlama-13B-FT}} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
 & \multicolumn{2}{c}{Spider} & \multicolumn{2}{c}{Bird} & \multicolumn{2}{c}{Spider} & \multicolumn{2}{c}{Bird} & \multicolumn{2}{c}{Spider} & \multicolumn{2}{c}{Bird} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}\cmidrule(lr){12-13}
 & Acc & H@1 & Acc & H@1 & Acc & H@1 & Acc & H@1 & Acc & H@1 & Acc & H@1 \\
\midrule
Naive & 58.2 & 57.0 & 49.4 & 12.7 & 67.0 & 59.0 & 64.3 & 16.0 & 69.7 & 61.3 & 62.1 & 16.0 \\
\midrule
+ Exec. Check & 78.7 & 62.8 & 78.8 & \textbf{20.0} & 84.8 & 64.0 & 86.3 & 22.0 & 83.6 & 65.3 & 82.2 & \textbf{21.3} \\
+ Exec. Result & 82.6 & 65.0 & \textbf{79.9} & 18.7 & 89.2 & 67.0 & 88.5 & 22.0 & 88.5 & \textbf{67.0} & \textbf{85.9} & 21.0 \\
+ Both & \textbf{83.6} & \textbf{65.3} & 79.6 & 18.7 & \textbf{90.0} & \textbf{67.3} & \textbf{89.2} & \textbf{22.3} & \textbf{88.5} & \textbf{67.0} & 85.1 & 21.0 \\
\midrule
Improvement & 20.5 & \underline{8.3} & \underline{30.5} & \underline{7.3} & \underline{23.0} & \underline{8.3} & 24.9 & 6.3 & 18.8 & 5.7 & 23.8 & 5.3 \\
\bottomrule
\end{tabular}
\vspace{-6pt}
\caption{\label{tab:text2sql_enhanced_llm}
Text2sql Enhanced Discriminator.
}
\vspace{-11pt}
\end{table*}
